3D Radiation hydrodynamics of a dynamical torus

We have developed a new dynamical model of the torus region in active galactic nucleus (AGN), using a three-dimensional radiation hydrodynamics algorithm. These new simulations have the specific aim to explore the role of radiatively-driven outflows, which is hotly debated in current literature as a possible explanation for the observed infrared emission from the polar regions of AGN. In this first paper, we only consider radiative effects induced by the primary radiation from the AGN. The simulations generate a disk & outflow structure that qualitatively agrees with observations, although the outflow is radial rather than polar, likely due to the lack of radiation pressure from hot dust. We find cut-offs between the wind and disk at gas temperatures of 1000 K and dust temperatures of 100 K, producing kinematic signatures that can be used for interpretation of high resolution infrared observations. We also produce line emission maps to aid in the interpretation of recent ALMA observations and future JWST observations. We investigate a number of simulation parameters, and find that the anisotropy of the radiation field is equally important to the Eddington factor, despite the anisotropy often being assumed to have a single sometimes arbitrary form in many previous works. We also find that supernovae can have a small but significant impact, but only at extremely high star formation rates.

==> natbib/README <==
                                 What is NATBIB?
                                 
It is a LaTeX (2e, with some support for 2.09) package to act as generalized
interface for standard and non-standard bibliographic style files (BibTeX).

It is intended primarily to produce author-year style citations from a variety
of non-standard .bst outputs; it therefore replaces the special and individual
packages that go along with such .bst files:
   apalike.sty    for    apalike.bst et al.
   newapa.sty            newapa.bst, 
   chicago.sty           chicago.bst, named.bst et al.
   harvard.sty           agsm.bst, dcu.bst, kluwer.bst et al.
   astron.sty            astron.bst, apa.bst, humanbio.bst, et al.
   authordate<n>.sty     authordate<n>.bst, aaai-named.bst
   
The above .bst files may also be used with natbib to produce author-year or 
numerical citations, so that switching from author-year to numerical is only 
a matter of selecting an option. 

The standard .bst files (plain et al) and other numerical citation .bst files
are also understood, but they can produce only numerical citations.
Replacement .bst files
   plainnat.bst
   abbrvnat.bst
   unsrtnat.bst
are provided to produce the same formatting of the reference list as the
standard equivalent, but allowing both author-year and numerical citations.

See my parallel custom-bib system for generating customized bst files.

For installation instructions and more details, see README.vxx.

Patrick W. Daly
Max-Planck-Institut f\"ur Sonnensystemforschung
D-37191 Katlenburg-Lindau, Germany
E-mail: daly@mps.mpg.de

